Continual Learning for Text Classification with Information Disentanglement Based Regularization

Continual learning has become increasingly important as it enables NLP models to constantly learn and gain knowledge over time. Previous continual learning methods are mainly designed to preserve knowledge from previous tasks, without much emphasis on how to well generalize models to new tasks. In this work, we propose an information disentanglement based regularization method for continual learning on text classification. Our proposed method first disentangles text hidden spaces into representations that are generic to all tasks and representations specific to each individual task, and further regularizes these representations differently to better constrain the knowledge required to generalize. We also introduce two simple auxiliary tasks: next sentence prediction and task-id prediction, for learning better generic and specific representation spaces. Experiments conducted on large-scale benchmarks demonstrate the effectiveness of our method in continual text classification tasks with various sequences and lengths over state-of-the-art baselines. We have publicly released our code at https://github.com/GT-SALT/IDBR.

==> comments.tex <==

% Artificial intelligence(AI) has outperformed human in a wide range of tasks, in which models only need to handle static data distributions. However, their ability to learn on changing data distributions and sequences of tasks continually is still far behind human: Unlike humans can easily reuse and maintain previous knowledge while learning new tasks, current machine learning models suffer from catastrophic forgetting \citep{mccloskey1989catastrophic}: while learning on new tasks, model's performance on previous learned tasks degrades rapidly and dramatically. This discrepancy is a vital gap between  state-of-the-art AI models and artificial general intelligence. To narrow this gap, continual learning \citep{ring1998child}, also known as lifelong learning \citep{thrun1998lifelong}, aims at developing models that can keep learning knowledge from emerging new tasks without having catastrophic forgetting on old tasks and even let the new knowledge and old knowledge benefit from each other \citep{lopez2017gradient}.

%To address this problem, continual learning\citep{ring1998child}, also known as lifelong learning\citep{thrun1998lifelong}, tried to develop models that can keep learning knowledge from emerging new tasks without having catastrophic forgetting on old tasks, or even let the new knowledge and old knowledge benefit from each other\citep{lopez2017gradient}. This research direction can further narrow the gap between machine learning and human learning, let us move one step closer to General Artificial Intelligence.

%since many researchers\citep{wang2019sentence, sun2019lamol, wang2020efficient} consistently find that simple examples replay can outperform popular regularization-based methods, such as EWC\citep{kirkpatrick2017overcoming}, GEM\citep{lopez2017gradient}, and MAS\citep{aljundi2018memory}. Since the number of saved examples in memory is usually small(for example 1\%), constantly training models on these examples while training on new tasks may lead to overfitting\citep{han2020continual}.

%Until now, a lot of methods have been explored in continual learning field, especially in Computer Vision\citep{rusu2016progressive, lopez2017gradient, li2017learning, aljundi2018memory, mallya2018packnet, javed2019meta}. Comparing to computer vision, continual learning in natural language processing has not been extensively explored, and most of proposed methods is built on examples replay: train current model with both examples from current task and examples from previous tasks. Previous examples can be saved in episodic memory \citep{wang2019sentence, d2019episodic} or generated by generative models \citep{sun2019lamol}. On the basis of example replay, representation alignment\citep{wang2019sentence} can mitigate previous representation distortion while learning new tasks, meta learning \citep{obamuyide2019meta, holla2020meta} is helpful to learn a robust initialization that is hard to forget, local adaptation\citep{d2019episodic, wang2020efficient} adapts model during inference using $K$ nearest neighbor in episodic memory.

% \jiaao{We might focus on NLP CL in the introduction. This could be discussed in the related work.}


%Despite the effectiveness for CV tasks, they often fail to work well when dealing with languages \citep{wang2019sentence, sun2019lamol, wang2020efficient}.
%Until now, various methods have been explored in continual learning field, especially in Computer Vision \citep{rusu2016progressive, lopez2017gradient, li2017learning, aljundi2018memory, mallya2018packnet, javed2019meta}. However, those methods which has been demonstrated effective in computer vision, such as EWC \citep{kirkpatrick2017overcoming}, GEM \citep{lopez2017gradient}, and MAS \citep{aljundi2018memory}, fail to work well in NLP field \citep{wang2019sentence, sun2019lamol, wang2020efficient}. 
% One reason for their failure could be attributed to the wide usage of large pretrained models \citep{devlin2018bert, radford2019language} in NLP: Being designed to maintain previous tasks' knowledge only, they are not good at mitigating the forgetting of those extensive general knowledge learned during pre-training, which is actually the basis of achieving promising results in any NLP task today. While finetuning continually, pretrained parameters are easily trivialized to new specific tasks \citep{yogatama2019learning}, making it difficult to maintain performance on previous tasks. \jiaao{The reason need to be reconsidered. Not convincing, the methods mentioned above could be directly applied to languages.}
% In NLP field, 


% A general direction in continual learning is to preserve previous knowledge while learning new knowledge, most of prior researches following this direction can be categorized into two classes: (i) treat previous knowledge as a whole and try to preserve all of them \citep{rebuffi2017icarl, wang2019sentence}. (ii) evaluate parameter's importance accoring to current model and try to preserve those important parameters \citep{lopez2017gradient, zenke2017continual, aljundi2018memory}. In fact, in the process of learning a sequence of tasks, there exists general knowledge which is beneficial to every task and not likely to change task-specific knowledge which may constantly change.

% In this work, we take a closer look at continual learning on text classification, which is one of the most fundamental tasks in natural language processing and has broad applications in real-world settings. Existing continual learning methods on languages are mainly (i) replay-based methods \cite{d2019episodic,sun2019lamol} \jiaao{Are there more related works here?} where examples from previous tasks are stored and re-trained during the learning of the current task to retain old information, or (ii) regularization-based methods \cite{wang2019sentence, han2020continual} where model parameters are directly constrained from changing to preserve previous knowledge. 
% In fact, all continual learning methods in NLP need previous example. 
% Category could be summarized as (i) Pure replay, where examples from previous tasks are stored and re-trained during the learning of the current task to retain old information (ii) Regularization-based replay, previous examples are further leveraged to add constraint on hidden space.
% Could be organized as follow:
% The former methods only leverage previous examples for re-training and usually store extensive data from seen tasks \cite{d2019episodic} or train language models based on task identifiers to generate numerous examples \cite{sun2019lamol}, which greatly increase the costs of memory and training time. Even though the latter more fully and efficiently utilize previous examples by manipulating hidden space on the basis of them, they generally view the whole hidden space equally important and regularize them to the same extent \cite{wang2019sentence}, thus limiting the performances on new tasks. We argue that only task-general parameters should be restrained from changing while task-specific parameters could be allowed to update to fit in different tasks.
% Replay-based methods usually store extensive data from seen tasks \cite{d2019episodic} or train language models based on task identifiers to generate numerous examples \cite{sun2019lamol}, which greatly increase the costs of memory and training time. Even though the Regularization-based methods escapes from hoarding seen data by directly manipulating model parameters, they generally view all the parameters equally important and regularize them to the same extent \cite{wang2019sentence}, thus limiting the performances on new tasks. We argue that only task-general parameters should be restrained from changing while task-specific parameters could be allowed to update to fit in different tasks.


%in which examples from previous tasks are directly leveraged to mitigate forgetting on previous tasks. 
% However, to preserve previous knowledge as much as possible, they either require storing and replaying all the data from previous tasks which greatly increases the costs of storing space \cite{d2019episodic}, or train language models based on task identifiers to generate numerous examples for replaying which tasks up significantly more training time \cite{sun2019lamol}. Such limitations make it unrealistic to be applied into real-world settings. 

%However, all those proposed methods have their own limitations. MbPA++ \citep{d2019episodic} stores huge amounts of examples from all the tasks and employs local adaptation, which costs longer time during inference, LAMOL \citep{sun2019lamol} requires more training time and resources since they are training a language model together with the Q\&A model for text classification. It also need task identifier during inference, which is unrealistic in the real-world setting.


%(1) We propose a regularization-based information disentanglement method for continual learning on text classification to better preserve common knowledge and adapt specific knowledge. (2) We combine regularization-based with a small amount of replaying examples achieved by strategic sampling. (3) We perform experiments to demonstrate the effectiveness of our proposed methods compared to state-of-the-art baselines. 


% where we endow deep learning models with continual learning abilities via regularizing model parameters with only a limit amount of relayed examples. Specifically, 



%In this paper, we propose a regularization-based information disentanglement method for continual learning, in which we utilize two supervised loss to create a general hidden space and a task-specific hidden space, add regularization on both of them separately. 


%Prior regularization-based methods either treat previous knowledge as a whole and try to preserve all of them \citep{rebuffi2017icarl, wang2019sentence}, or evaluate parameter's importance and try to preserve those important parameters \citep{lopez2017gradient, zenke2017continual, aljundi2018memory}. 


%By disentangling information that is general to all tasks and information that is specific to individual tasks, we can give flexible and different regularization on each part. The learned general space can facilitate future learning on new tasks and the task-specific space explicitly maintain a capacity for future task-specific features. Our experiments show that our regularization-based information disentanglement is effective enough to outperform strong baselines and achieve comparable results to previous State-of-the-art approaches.

% \xuezhi{short bullet point summary for contribution}



%\jiaao{The story could be focusing on disentanglement, LM/NSP are just ways to do the disentangle general space, be orthogonal to other objectives}

%\jiaao{1. Might need to state what is continual learning, we need continual learning in the first paragraph.}


%\jiaao{2. Then briefly talked about previous methods in CV field, can they be directly applied to NLP? Has not been explored seems not a good need. Might need a stronger reason to state why we need to explore continual learning specifically for NLP, could start with discussing current large pre-trained models store extensive world/commonsense/general knowledge [cite some work here] (this might be a discrepency compared to CV settings), and fine-tuning is the mostly used methods for all sorts of tasks, however would cause forgetting general knowledge in previous models, which prevent xxx.  }


%\jiaao{3. Next discuss previous efforts in NLP fields, what are their corresponding limitations? e.g., store significant more data/require more resources/cost longer time during inference/overfit on replayed example. }


%\jiaao{4. To overcome these limitations, we propose xxxxxx. and describe the intuition behind the model design. }


% The learning ability of human-being has evolved to handle the non-stationary of this world, which is robust to changing tasks and sequential experience\citep{hadsell2020embracing}. However, even though current artificial intelligence has outperformed human in a wide range of tasks, their ability to learn a sequence of tasks continually is still far behind human, mainly due to catastrophic forgetting\citep{mccloskey1989catastrophic}: while learning on current task, model's performance on previous learned tasks degrades rapidly and dramatically. 

% could state following: 
% What is continual Learning
% Previous regularized methods regularize the change of all the parameters/space to the same extent while we claim that there are xxx and xxx in large hidden space, and xxx does need to change across different task
% To this end, we present xxx 
% Experiments showed that xxx

% that is general to all tasks and information that is specific to each individual task, 
% we can better preserve the knowledge required to learn and generalize, which helps alleviate the problem of catastrophic forgetting.


% We argue that only task-general parameters should be restrained from changing while task-specific parameters could be allowed to update to fit in different tasks.
% However, methods that are effective in CV tasks often fail to work well when dealing with languages \citep{wang2019sentence, sun2019lamol, wang2020efficient}. One reason for their failure could be attributed to the wide usage of large pretrained models \citep{devlin2018bert, radford2019language} in NLP: Being designed to maintain previous tasks' knowledge only, they are not good at mitigating the forgetting of those extensive general knowledge learned during pre-training, which is actually the basis of achieving promising results in any NLP task today. While finetuning continually, pretrained parameters are easily trivialized to new specific tasks \citep{yogatama2019learning}, making it difficult to maintain performance on previous tasks. 
% Take a closer look at proposed methods in continual learning for NLP, all of them has their limitations. For example, Pure replay methods usually store extensive data from seen tasks \cite{d2019episodic} or train language models based on task identifiers to generate numerous examples \cite{sun2019lamol}, which greatly increase the costs of memory and training time. Even though the Regularization-based replay methods more fully and efficiently utilize previous examples by manipulating hidden space on the basis of them, they generally view the whole hidden space equally important and regularize them to the same extent \cite{wang2019sentence}, thus limiting the performances on new tasks. We argue that only task-general parameters should be restrained from changing while task-specific parameters could be allowed to update to fit in different tasks.


% Our proposed model can be viewed as a combination of the replay-based method and regularization-based method, which preserves knowledge via re-training on sampled examples from previous tasks and regularizing model's output from changing too much.
% Our method could be considered as a hybrid method 
% : we use a episodic memory to store examples from previous tasks in order to facilitate information disentanglement, as well as we employ regularization on hidden space to prevent severe distortion.

% \paragraph{Continual Leaning for NLP} Continual leaning for text has received growing attention recently with the trend of adapting large pre-trained models \cite{devlin2018bert,radford2019language} on all kinds of NLP tasks, which enable pre-trained models continually acquire novel world knowledge from streams of textual data without forgetting already learned knowledge. 


% Extensive efforts have been focused on purely replaying 

% d2019episodic,sun2019lamol,holla2020meta


%For continual learning in NLP, \citet{wang2019sentence} firstly use episodic memory replay for continual relation extraction, in which they utilize representation alignment to mitigate representation distortion. Using the same architecture, \citet{obamuyide2019meta} combine experience replay with Reptile \citep{nichol2018first}, and \citet{han2020continual} further introduce  episodic memory activation and reconsolidation to mitigate overfitting on saved examples. \citet{d2019episodic} leverage sparse memory replay during training and local adaptation using $K$ nearest neighbor during inference on text classification and question answering, put forward MbPA++. \citet{wang2020efficient} improve MbPA++ by using meta learning to learn a generic representation for local adaptation and select examples in memory by diversity. \citet{sun2019lamol} treat all kinds of NLP tasks as question answering \citep{mccann2018natural} and propose LAMOL, which learn to solve current task and generate current task's examples simultaneously while generating pseudo examples from previous tasks for replay before training on any new task. %\jiaao{What are their limitations? Why we proposed our methods?}


% \section{Approach}


% In this section, we first introduce the formal definition and some background information for continual learning in Section \ref{background}, then elaborate the high-level intuition and technical details of our method in Section \ref{our-method}.
%we present how we augment our model with an episodic memory module,  how we disentangle task-general information and task-specific information and how we apply regularization on the hidden space.


%We introduce the definition of continual learning and the detailed setting for our task. Besides, background information for the episodic module used in our model is given.



% \xuezhi{the two notations of T and $\mathcal{T}$ need to be consistent, which one do you intend to use?}
%The goal of continual learning is to design a model which can perform well on the new tasks which preserving knowledge of old tasks. Specifically, we study the task-incremental continual learning. Formally, task-incremental continual learning is defined as follows: given a task sequence with $T$ tasks, design a model which has best average performance on all $T$ tasks after being trained on them one after one. In task-incremental learning, both the domain and label space of each task are not guaranteed to be same. Let the domain, label space, distribution of $T$ tasks be  $\{ \mathcal{X}^t \}_{t=1}^{T}$, $\{ \mathcal{Y}^t \}_{t=1}^{T}$, $\{\mathcal{D}^t \}_{t=1}^{T}$. For the text classification task we study, we want to learn a classifier learn a classifier $f_\theta : \bigcup_{i=1}^{T} \mathcal{X}^t \to \bigcup_{i=1}^{T} \mathcal{Y}^t $ minimizing the generalization error on the $T$ tasks:
%\begin{equation*}
%    \begin{split}
%        R(f_\theta) = \sum_{t=1}^{T} \mathbb{E}_{(x, y) \sim \mathcal{D}^t} %\mathcal{L}(f_\theta(x), y) 
%    \end{split}
%\end{equation*}


% This is usually achieved by adding a penalty term between old features and new features.
% In practice, every time before learning a new task, regularization-based methods store those old features first. After training start,  is added  to mitigate severe change.
% The intuition behind regularization-based method \citep{li2017learning, rannen2017encoder, lopez2017gradient, zenke2017continual, aljundi2018memory, wang2019sentence} is to add constraints while learning new tasks, preventing it from disturbing previous knowledge. Regularization-based methods commonly store vital information before training on new tasks, then constraints are added to prevent those information from changing a lot during subsequent training.
% \paragraph{Task Settings}


% \paragraph{Replay-Based Methods} Experience Replay is a commonly used method in CL for NLP. This kind of method will augment the model with a memory buffer $\mathcal{M}$ which stores seen examples from previous tasks. By replaying stored examples from previous tasks, it helps the model to recall previous knowledge. Our model is augmented with $\mathcal{M}$ as well. Let $\mathcal{M}^t$ be the memory module before training on task $t$. The initial $\mathcal{M}^1$ is empty. After training on task $t$, we will select $\gamma n$ examples from the training set $S^t$ using KMeans where $n$ is the size of $S^t$ and $\gamma$ is the store ratio. Then we add these selected examples into $\mathcal{M}$ and get $\mathcal{M}^{t+1}$. 
